Low-Resource Syntactic Transfer with Unsupervised Source Reordering

We describe a cross-lingual transfer method for dependency parsing that takes into account the problem of word order differences between source and target languages. Our model only relies on the Bible, a considerably smaller parallel data than the commonly used parallel data in transfer methods. We use the concatenation of projected trees from the Bible corpus, and the gold-standard treebanks in multiple source languages along with cross-lingual word representations. We demonstrate that reordering the source treebanks before training on them for a target language improves the accuracy of languages outside the European language family. Our experiments on 68 treebanks (38 languages) in the Universal Dependencies corpus achieve a high accuracy for all languages. Among them, our experiments on 16 treebanks of 12 non-European languages achieve an average UAS absolute improvement of 3.3% over a state-of-the-art method.

==> dep_analysis.tex <==
\begin{table*}[t!]
\centering
    \tiny
     \renewcommand{\arraystretch}{0.5}
     \setlength{\tabcolsep}{5pt}
    \begin{tabular}{| l | l |  c | c | c | c | c | c | c  | c | c| c| c|  c|    }
    \hline
 lang & data & acl & advmod & amod & conj & nmod & nsubj & obj & obl & root\\ \hline 
ar & ar & \cellcolor{green!90.0} 33.6/35.4 & \cellcolor{green!15.0} 66.0/66.3 & \cellcolor{green!100} 80.4/84.0 & \cellcolor{green!60.0} 41.5/42.7 & \cellcolor{green!100} 60.8/63.8 & \cellcolor{red!100} 54.9/41.5 & \cellcolor{green!100} 54.6/69.8 & \cellcolor{green!100} 48.8/52.6 & \cellcolor{green!45.0} 29.3/30.2\\ 
ar & ar\_pud & \cellcolor{green!100} 37.1/42.3 & \cellcolor{red!65.0} 62.3/61.0 & \cellcolor{green!100} 74.1/80.9 & \cellcolor{green!50.0} 48.2/49.2 & \cellcolor{green!100} 66.0/69.1 & \cellcolor{red!100} 61.3/58.6 & \cellcolor{green!100} 69.8/78.7 & \cellcolor{green!100} 51.1/55.1 & \cellcolor{green!100} 63.5/67.4\\ 
bg & bg & \cellcolor{green!60.0} 61.7/62.9 & \cellcolor{green!30.0} 77.0/77.6 & \cellcolor{green!10.0} 92.1/92.3 & \cellcolor{red!20.0} 67.8/67.4 & \cellcolor{green!55.0} 75.4/76.5 & \cellcolor{red!20.0} 84.9/84.5 & \cellcolor{green!5.0} 92.8/92.9 & \cellcolor{red!5.0} 79.4/79.3 & \cellcolor{red!20.0} 82.3/81.9\\ 
cop & cop & \cellcolor{green!100} 12.1/28.6 & \cellcolor{red!50.0} 64.5/63.5 & \cellcolor{green!100} 50.0/80.0 & \cellcolor{red!100} 32.1/22.2 & \cellcolor{green!100} 44.0/52.9 & \cellcolor{green!50.0} 82.2/83.2 & \cellcolor{red!100} 66.7/64.5 & \cellcolor{green!100} 56.3/67.8 & \cellcolor{green!0.0} 60.6/60.6\\ 
cs & cs & \cellcolor{green!25.0} 49.7/50.2 & \cellcolor{green!10.0} 68.9/69.1 & \cellcolor{green!20.0} 89.4/89.8 & \cellcolor{green!25.0} 57.1/57.6 & \cellcolor{green!90.0} 63.6/65.4 & \cellcolor{green!40.0} 71.3/72.1 & \cellcolor{green!0.0} 78.2/78.2 & \cellcolor{green!15.0} 70.5/70.8 & \cellcolor{green!10.0} 79.8/80.0\\ 
cs & cs\_cac & \cellcolor{green!50.0} 52.5/53.5 & \cellcolor{red!55.0} 66.7/65.6 & \cellcolor{green!20.0} 89.1/89.5 & \cellcolor{green!0.0} 61.9/61.9 & \cellcolor{green!90.0} 66.1/67.9 & \cellcolor{green!70.0} 72.6/74.0 & \cellcolor{green!0.0} 79.9/79.9 & \cellcolor{green!30.0} 72.2/72.8 & \cellcolor{green!25.0} 79.6/80.1\\ 
cs & cs\_cltt & \cellcolor{red!15.0} 49.6/49.3 & \cellcolor{green!30.0} 44.9/45.5 & \cellcolor{green!20.0} 89.4/89.8 & \cellcolor{red!25.0} 46.7/46.2 & \cellcolor{green!100} 60.0/63.2 & \cellcolor{green!60.0} 70.3/71.5 & \cellcolor{green!5.0} 76.8/76.9 & \cellcolor{green!85.0} 57.5/59.2 & \cellcolor{red!30.0} 76.7/76.1\\ 
cs & cs\_pud & \cellcolor{green!35.0} 53.2/53.9 & \cellcolor{red!30.0} 71.4/70.8 & \cellcolor{green!20.0} 89.5/89.9 & \cellcolor{green!25.0} 64.4/64.9 & \cellcolor{green!85.0} 62.1/63.8 & \cellcolor{green!25.0} 76.4/76.9 & \cellcolor{green!15.0} 83.3/83.6 & \cellcolor{green!5.0} 72.5/72.6 & \cellcolor{red!15.0} 83.5/83.2\\ 
da & da & \cellcolor{green!50.0} 51.9/52.9 & \cellcolor{red!60.0} 70.8/69.6 & \cellcolor{green!20.0} 84.5/84.9 & \cellcolor{red!15.0} 69.1/68.8 & \cellcolor{red!30.0} 62.6/62.0 & \cellcolor{green!10.0} 83.7/83.9 & \cellcolor{green!25.0} 85.5/86.0 & \cellcolor{green!30.0} 60.4/61.0 & \cellcolor{red!75.0} 75.0/73.5\\ 
de & de & \cellcolor{red!100} 41.8/39.4 & \cellcolor{green!20.0} 63.9/64.3 & \cellcolor{green!75.0} 85.7/87.2 & \cellcolor{green!25.0} 62.0/62.5 & \cellcolor{green!35.0} 64.8/65.5 & \cellcolor{green!25.0} 76.2/76.7 & \cellcolor{green!50.0} 76.8/77.8 & \cellcolor{green!90.0} 67.5/69.3 & \cellcolor{red!5.0} 79.3/79.2\\ 
de & de\_pud & \cellcolor{red!75.0} 52.6/51.1 & \cellcolor{green!55.0} 64.9/66.0 & \cellcolor{green!50.0} 86.5/87.5 & \cellcolor{green!55.0} 61.8/62.9 & \cellcolor{red!25.0} 70.8/70.3 & \cellcolor{green!55.0} 81.1/82.2 & \cellcolor{green!35.0} 80.8/81.5 & \cellcolor{green!10.0} 68.5/68.7 & \cellcolor{red!10.0} 83.0/82.8\\ 
el & el & \cellcolor{green!95.0} 40.0/41.9 & \cellcolor{green!0.0} 73.1/73.1 & \cellcolor{green!80.0} 83.7/85.3 & \cellcolor{red!10.0} 55.8/55.6 & \cellcolor{green!90.0} 59.0/60.8 & \cellcolor{green!45.0} 71.0/71.9 & \cellcolor{red!20.0} 85.4/85.0 & \cellcolor{green!35.0} 67.5/68.2 & \cellcolor{red!25.0} 77.9/77.4\\ 
en & en & \cellcolor{green!55.0} 49.2/50.3 & \cellcolor{red!10.0} 77.2/77.0 & \cellcolor{green!50.0} 76.8/77.8 & \cellcolor{green!5.0} 64.4/64.5 & \cellcolor{green!5.0} 54.2/54.3 & \cellcolor{red!5.0} 80.7/80.6 & \cellcolor{green!30.0} 80.5/81.1 & \cellcolor{green!30.0} 64.6/65.2 & \cellcolor{red!10.0} 80.9/80.7\\ 
en & en\_lines & \cellcolor{green!75.0} 59.9/61.4 & \cellcolor{green!15.0} 72.2/72.5 & \cellcolor{green!0.0} 83.4/83.4 & \cellcolor{green!50.0} 63.8/64.8 & \cellcolor{green!20.0} 64.5/64.9 & \cellcolor{green!15.0} 83.1/83.4 & \cellcolor{green!45.0} 85.3/86.2 & \cellcolor{green!20.0} 74.9/75.3 & \cellcolor{green!10.0} 81.8/82.0\\ 
en & en\_partut & \cellcolor{green!65.0} 51.6/52.9 & \cellcolor{green!35.0} 72.9/73.6 & \cellcolor{green!80.0} 84.1/85.7 & \cellcolor{green!10.0} 60.1/60.3 & \cellcolor{green!0.0} 58.7/58.7 & \cellcolor{red!25.0} 82.0/81.5 & \cellcolor{green!40.0} 80.7/81.5 & \cellcolor{green!35.0} 70.9/71.6 & \cellcolor{red!15.0} 87.0/86.7\\ 
en & en\_pud & \cellcolor{green!90.0} 56.3/58.1 & \cellcolor{green!5.0} 74.7/74.8 & \cellcolor{green!50.0} 79.9/80.9 & \cellcolor{green!15.0} 64.7/65.0 & \cellcolor{green!10.0} 65.7/65.9 & \cellcolor{green!25.0} 81.8/82.3 & \cellcolor{green!40.0} 82.3/83.1 & \cellcolor{green!0.0} 70.0/70.0 & \cellcolor{red!15.0} 86.9/86.6\\ 
es & es & \cellcolor{green!35.0} 59.7/60.4 & \cellcolor{green!35.0} 76.6/77.3 & \cellcolor{green!25.0} 88.3/88.8 & \cellcolor{green!45.0} 60.6/61.5 & \cellcolor{green!20.0} 77.8/78.2 & \cellcolor{green!25.0} 80.8/81.3 & \cellcolor{green!15.0} 91.1/91.4 & \cellcolor{green!10.0} 78.2/78.4 & \cellcolor{red!85.0} 82.2/80.5\\ 
es & es\_ancora & \cellcolor{red!40.0} 58.0/57.2 & \cellcolor{red!65.0} 72.5/71.2 & \cellcolor{green!5.0} 88.7/88.8 & \cellcolor{red!5.0} 64.2/64.1 & \cellcolor{green!15.0} 79.0/79.3 & \cellcolor{red!5.0} 86.2/86.1 & \cellcolor{green!5.0} 86.9/87.0 & \cellcolor{green!0.0} 74.2/74.2 & \cellcolor{red!60.0} 86.4/85.2\\ 
es & es\_pud & \cellcolor{green!40.0} 57.9/58.7 & \cellcolor{red!100.0} 72.6/70.6 & \cellcolor{red!5.0} 91.0/90.9 & \cellcolor{green!20.0} 68.8/69.2 & \cellcolor{green!5.0} 81.0/81.1 & \cellcolor{green!5.0} 85.7/85.8 & \cellcolor{red!10.0} 93.5/93.3 & \cellcolor{green!40.0} 74.1/74.9 & \cellcolor{green!30.0} 84.9/85.5\\ 
et & et & \cellcolor{red!60.0} 48.5/47.3 & \cellcolor{red!20.0} 69.3/68.9 & \cellcolor{green!45.0} 73.6/74.5 & \cellcolor{green!30.0} 54.1/54.7 & \cellcolor{red!35.0} 63.6/62.9 & \cellcolor{red!20.0} 75.5/75.1 & \cellcolor{green!10.0} 76.6/76.8 & \cellcolor{red!95.0} 44.5/42.6 & \cellcolor{green!30.0} 73.1/73.7\\ 
eu & eu & \cellcolor{green!100} 2.6/4.9 & \cellcolor{green!45.0} 56.3/57.2 & \cellcolor{red!80.0} 64.3/62.7 & \cellcolor{green!100} 36.9/40.9 & \cellcolor{green!100} 19.6/49.1 & \cellcolor{green!100} 51.5/61.9 & \cellcolor{green!100} 44.9/60.3 & \cellcolor{green!100} 13.1/26.5 & \cellcolor{green!100} 54.0/58.7\\ 
fa & fa & \cellcolor{green!100} 39.0/46.3 & \cellcolor{green!100} 40.9/45.8 & \cellcolor{green!100} 79.3/81.7 & \cellcolor{green!100} 42.2/44.6 & \cellcolor{green!100} 64.1/66.8 & \cellcolor{green!100} 45.4/52.5 & \cellcolor{green!100} 58.2/67.0 & \cellcolor{green!100} 55.7/64.3 & \cellcolor{green!100} 59.2/63.3\\ 
fi & fi & \cellcolor{red!100.0} 46.1/44.1 & \cellcolor{green!10.0} 61.8/62.0 & \cellcolor{green!65.0} 78.7/80.0 & \cellcolor{green!35.0} 60.1/60.8 & \cellcolor{green!100} 54.1/56.3 & \cellcolor{green!55.0} 70.7/71.8 & \cellcolor{red!60.0} 70.1/68.9 & \cellcolor{red!80.0} 58.9/57.3 & \cellcolor{red!15.0} 72.9/72.6\\ 
fi & fi\_ftb & \cellcolor{red!75.0} 38.5/37.0 & \cellcolor{green!30.0} 62.2/62.8 & \cellcolor{green!35.0} 77.4/78.1 & \cellcolor{green!25.0} 56.4/56.9 & \cellcolor{green!75.0} 42.3/43.8 & \cellcolor{green!10.0} 72.3/72.5 & \cellcolor{red!55.0} 73.4/72.3 & \cellcolor{green!40.0} 75.3/76.1 & \cellcolor{green!25.0} 72.0/72.5\\ 
fi & fi\_pud & \cellcolor{green!15.0} 50.2/50.5 & \cellcolor{green!25.0} 65.4/65.9 & \cellcolor{green!40.0} 79.2/80.0 & \cellcolor{green!55.0} 63.5/64.6 & \cellcolor{green!50.0} 58.7/59.7 & \cellcolor{green!30.0} 72.7/73.3 & \cellcolor{green!20.0} 70.4/70.8 & \cellcolor{red!30.0} 64.4/63.8 & \cellcolor{green!45.0} 76.9/77.8\\ 
fr & fr & \cellcolor{green!45.0} 53.8/54.7 & \cellcolor{green!30.0} 75.0/75.6 & \cellcolor{green!0.0} 88.5/88.5 & \cellcolor{red!5.0} 62.3/62.2 & \cellcolor{green!35.0} 76.5/77.2 & \cellcolor{green!0.0} 85.8/85.8 & \cellcolor{green!60.0} 89.4/90.6 & \cellcolor{green!65.0} 69.3/70.6 & \cellcolor{green!15.0} 81.0/81.3\\ 
fr & fr\_partut & \cellcolor{green!100} 57.3/61.1 & \cellcolor{green!25.0} 77.8/78.3 & \cellcolor{red!20.0} 87.8/87.4 & \cellcolor{green!15.0} 61.9/62.2 & \cellcolor{green!40.0} 76.2/77.0 & \cellcolor{green!10.0} 84.2/84.4 & \cellcolor{green!15.0} 90.9/91.2 & \cellcolor{green!60.0} 73.1/74.3 & \cellcolor{green!70.0} 84.0/85.4\\ 
fr & fr\_pud & \cellcolor{green!10.0} 66.3/66.5 & \cellcolor{red!20.0} 74.2/73.8 & \cellcolor{green!10.0} 89.9/90.1 & \cellcolor{green!10.0} 67.3/67.5 & \cellcolor{green!0.0} 77.6/77.6 & \cellcolor{green!15.0} 83.2/83.5 & \cellcolor{green!5.0} 92.7/92.8 & \cellcolor{green!25.0} 72.8/73.3 & \cellcolor{red!35.0} 84.6/83.9\\ 
fr & fr\_sequoia & \cellcolor{red!25.0} 53.2/52.7 & \cellcolor{green!25.0} 71.6/72.1 & \cellcolor{red!5.0} 90.5/90.4 & \cellcolor{red!5.0} 60.8/60.7 & \cellcolor{red!5.0} 77.0/76.9 & \cellcolor{red!50.0} 82.9/81.9 & \cellcolor{green!10.0} 91.6/91.8 & \cellcolor{green!10.0} 70.9/71.1 & \cellcolor{green!30.0} 84.8/85.4\\ 
he & he & \cellcolor{green!45.0} 40.7/41.6 & \cellcolor{green!90.0} 53.1/54.9 & \cellcolor{green!85.0} 77.1/78.8 & \cellcolor{green!100} 48.2/51.1 & \cellcolor{green!100} 72.1/75.3 & \cellcolor{green!100} 60.2/65.3 & \cellcolor{green!20.0} 76.8/77.2 & \cellcolor{green!95.0} 69.2/71.1 & \cellcolor{green!15.0} 63.3/63.6\\ 
hi & hi & \cellcolor{green!55.0} 43.5/44.6 & \cellcolor{red!100} 58.0/50.4 & \cellcolor{green!10.0} 75.4/75.6 & \cellcolor{red!100} 40.5/38.3 & \cellcolor{red!15.0} 65.7/65.4 & \cellcolor{green!100.0} 47.3/49.3 & \cellcolor{red!25.0} 70.3/69.8 & \cellcolor{green!100} 50.8/53.4 & \cellcolor{red!30.0} 68.8/68.2\\ 
hi & hi\_pud & \cellcolor{green!0.0} 28.1/28.1 & \cellcolor{green!85.0} 50.6/52.3 & \cellcolor{red!5.0} 75.6/75.5 & \cellcolor{green!55.0} 39.5/40.6 & \cellcolor{green!45.0} 64.8/65.7 & \cellcolor{green!65.0} 49.5/50.8 & \cellcolor{green!90.0} 59.4/61.2 & \cellcolor{green!100} 48.9/51.2 & \cellcolor{green!100} 56.5/58.9\\ 
hr & hr & \cellcolor{green!0.0} 56.5/56.5 & \cellcolor{green!25.0} 71.2/71.7 & \cellcolor{green!5.0} 90.4/90.5 & \cellcolor{green!65.0} 64.1/65.4 & \cellcolor{green!30.0} 76.5/77.1 & \cellcolor{green!30.0} 78.9/79.5 & \cellcolor{green!35.0} 87.3/88.0 & \cellcolor{green!40.0} 73.7/74.5 & \cellcolor{green!100} 79.3/81.5\\ 
hu & hu & \cellcolor{red!100} 32.8/30.2 & \cellcolor{green!10.0} 69.6/69.8 & \cellcolor{green!45.0} 82.4/83.3 & \cellcolor{green!20.0} 52.1/52.5 & \cellcolor{green!100} 44.4/49.0 & \cellcolor{green!50.0} 71.5/72.5 & \cellcolor{red!10.0} 79.0/78.8 & \cellcolor{green!50.0} 72.9/73.9 & \cellcolor{red!15.0} 69.3/69.0\\ 
id & id & \cellcolor{green!15.0} 45.6/45.9 & \cellcolor{green!100.0} 77.9/79.9 & \cellcolor{green!100} 59.2/74.0 & \cellcolor{green!70.0} 56.1/57.5 & \cellcolor{green!100} 73.3/77.8 & \cellcolor{green!100} 80.0/82.2 & \cellcolor{green!100} 81.1/85.3 & \cellcolor{green!100} 73.4/77.4 & \cellcolor{green!40.0} 82.9/83.7\\ 
it & it & \cellcolor{red!50.0} 65.4/64.4 & \cellcolor{green!90.0} 74.3/76.1 & \cellcolor{green!45.0} 87.3/88.2 & \cellcolor{red!40.0} 61.2/60.4 & \cellcolor{green!0.0} 80.5/80.5 & \cellcolor{red!75.0} 80.1/78.6 & \cellcolor{green!40.0} 91.8/92.6 & \cellcolor{green!60.0} 75.2/76.4 & \cellcolor{red!40.0} 80.1/79.3\\ 
it & it\_pud & \cellcolor{green!0.0} 65.8/65.8 & \cellcolor{green!20.0} 78.2/78.6 & \cellcolor{green!5.0} 89.6/89.7 & \cellcolor{red!25.0} 67.3/66.8 & \cellcolor{green!10.0} 82.5/82.7 & \cellcolor{red!25.0} 87.7/87.2 & \cellcolor{green!15.0} 93.1/93.4 & \cellcolor{green!10.0} 77.6/77.8 & \cellcolor{red!30.0} 87.5/86.9\\ 
ja & ja & \cellcolor{green!85.0} 19.6/21.3 & \cellcolor{red!5.0} 66.2/66.1 & \cellcolor{red!100} 67.4/63.3 & \cellcolor{red!45.0} 2.1/1.2 & \cellcolor{green!50.0} 72.7/73.7 & \cellcolor{green!15.0} 51.6/51.9 & \cellcolor{green!100} 80.1/86.3 & \cellcolor{green!100} 64.9/67.5 & \cellcolor{green!15.0} 35.8/36.1\\ 
ja & ja\_pud & \cellcolor{green!100} 23.9/27.9 & \cellcolor{green!100} 58.5/60.8 & \cellcolor{red!100} 70.1/66.9 & \cellcolor{green!10.0} 1.2/1.4 & \cellcolor{green!15.0} 68.4/68.7 & \cellcolor{green!100} 50.7/53.0 & \cellcolor{green!100} 82.8/86.6 & \cellcolor{green!80.0} 62.6/64.2 & \cellcolor{red!100} 41.2/38.4\\ 
ko & ko & \cellcolor{green!100} 39.4/43.3 & \cellcolor{green!75.0} 58.9/60.4 & \cellcolor{green!100} 71.9/77.7 & \cellcolor{green!100} 15.8/19.3 & \cellcolor{green!55.0} 24.4/25.5 & \cellcolor{red!95.0} 40.0/38.1 & \cellcolor{green!95.0} 67.2/69.1 & \cellcolor{green!45.0} 58.1/59.0 & \cellcolor{red!60.0} 66.3/65.1\\ 
la & la & \cellcolor{red!50.0} 28.6/27.6 & \cellcolor{green!30.0} 56.3/56.9 & \cellcolor{red!5.0} 34.6/34.5 & \cellcolor{red!45.0} 41.5/40.6 & \cellcolor{green!95.0} 34.6/36.5 & \cellcolor{green!75.0} 63.8/65.3 & \cellcolor{red!100} 63.5/61.2 & \cellcolor{red!100} 67.4/63.8 & \cellcolor{red!15.0} 70.6/70.3\\ 
la & la\_ittb & \cellcolor{green!20.0} 38.0/38.4 & \cellcolor{green!5.0} 65.2/65.3 & \cellcolor{green!0.0} 69.4/69.4 & \cellcolor{red!35.0} 51.1/50.4 & \cellcolor{green!100.0} 49.0/51.0 & \cellcolor{green!65.0} 60.0/61.3 & \cellcolor{red!45.0} 68.9/68.0 & \cellcolor{green!65.0} 59.3/60.6 & \cellcolor{green!0.0} 67.6/67.6\\ 
la & la\_proiel & \cellcolor{green!40.0} 43.1/43.9 & \cellcolor{green!15.0} 63.5/63.8 & \cellcolor{green!15.0} 62.2/62.5 & \cellcolor{red!5.0} 52.2/52.1 & \cellcolor{red!45.0} 66.0/65.1 & \cellcolor{green!55.0} 65.6/66.7 & \cellcolor{red!30.0} 73.7/73.1 & \cellcolor{red!40.0} 68.1/67.3 & \cellcolor{red!35.0} 70.0/69.3\\ 
lt & lt & \cellcolor{green!0.0} 33.3/33.3 & \cellcolor{red!25.0} 77.2/76.7 & \cellcolor{red!20.0} 72.2/71.8 & \cellcolor{green!100} 57.0/59.4 & \cellcolor{green!100} 78.4/80.8 & \cellcolor{red!10.0} 69.5/69.3 & \cellcolor{red!100} 67.1/64.3 & \cellcolor{red!60.0} 58.0/56.8 & \cellcolor{red!100} 67.3/63.6\\ 
lv & lv & \cellcolor{red!55.0} 37.1/36.0 & \cellcolor{green!60.0} 73.8/75.0 & \cellcolor{green!70.0} 65.7/67.1 & \cellcolor{green!65.0} 46.9/48.2 & \cellcolor{red!45.0} 47.9/47.0 & \cellcolor{green!45.0} 70.2/71.1 & \cellcolor{red!10.0} 69.4/69.2 & \cellcolor{red!60.0} 58.3/57.1 & \cellcolor{red!5.0} 72.6/72.5\\ 
nl & nl & \cellcolor{green!70.0} 43.9/45.3 & \cellcolor{green!20.0} 60.3/60.7 & \cellcolor{green!100.0} 84.7/86.7 & \cellcolor{green!20.0} 65.9/66.3 & \cellcolor{red!40.0} 65.8/65.0 & \cellcolor{green!10.0} 68.2/68.4 & \cellcolor{green!65.0} 57.4/58.7 & \cellcolor{green!65.0} 59.5/60.8 & \cellcolor{red!20.0} 67.9/67.5\\ 
nl & nl\_lassysmall & \cellcolor{red!25.0} 45.9/45.4 & \cellcolor{green!75.0} 73.0/74.5 & \cellcolor{green!5.0} 81.5/81.6 & \cellcolor{red!30.0} 69.0/68.4 & \cellcolor{red!30.0} 73.9/73.3 & \cellcolor{green!45.0} 76.2/77.1 & \cellcolor{green!20.0} 80.6/81.0 & \cellcolor{red!25.0} 69.2/68.7 & \cellcolor{green!50.0} 83.1/84.1\\ 
no & no\_bokmaal & \cellcolor{green!40.0} 62.9/63.7 & \cellcolor{red!5.0} 72.4/72.3 & \cellcolor{green!30.0} 89.2/89.8 & \cellcolor{green!15.0} 66.8/67.1 & \cellcolor{green!5.0} 69.5/69.6 & \cellcolor{red!5.0} 84.2/84.1 & \cellcolor{red!5.0} 89.0/88.9 & \cellcolor{green!0.0} 72.6/72.6 & \cellcolor{green!5.0} 81.3/81.4\\ 
no & no\_nynorsk & \cellcolor{green!75.0} 56.8/58.3 & \cellcolor{green!10.0} 62.4/62.6 & \cellcolor{green!50.0} 87.3/88.3 & \cellcolor{green!40.0} 66.0/66.8 & \cellcolor{green!40.0} 66.7/67.5 & \cellcolor{green!20.0} 78.1/78.5 & \cellcolor{red!10.0} 83.9/83.7 & \cellcolor{green!30.0} 64.5/65.1 & \cellcolor{green!15.0} 77.0/77.3\\ 
pl & pl & \cellcolor{green!10.0} 58.0/58.2 & \cellcolor{green!15.0} 78.1/78.4 & \cellcolor{green!45.0} 79.8/80.7 & \cellcolor{green!35.0} 68.9/69.6 & \cellcolor{green!50.0} 68.7/69.7 & \cellcolor{red!25.0} 75.3/74.8 & \cellcolor{red!5.0} 83.2/83.1 & \cellcolor{green!20.0} 78.8/79.2 & \cellcolor{red!25.0} 86.5/86.0\\ 
pt & pt & \cellcolor{green!25.0} 55.2/55.7 & \cellcolor{green!30.0} 72.4/73.0 & \cellcolor{red!25.0} 88.6/88.1 & \cellcolor{red!25.0} 67.3/66.8 & \cellcolor{green!5.0} 80.3/80.4 & \cellcolor{green!50.0} 80.9/81.9 & \cellcolor{green!0.0} 88.2/88.2 & \cellcolor{red!25.0} 76.3/75.8 & \cellcolor{red!40.0} 80.3/79.5\\ 
pt & pt\_br & \cellcolor{green!60.0} 55.7/56.9 & \cellcolor{green!10.0} 73.0/73.2 & \cellcolor{green!15.0} 84.8/85.1 & \cellcolor{green!5.0} 59.4/59.5 & \cellcolor{red!20.0} 68.1/67.7 & \cellcolor{green!10.0} 78.2/78.4 & \cellcolor{red!15.0} 91.1/90.8 & \cellcolor{green!45.0} 84.7/85.6 & \cellcolor{red!40.0} 75.0/74.2\\ 
pt & pt\_pud & \cellcolor{red!35.0} 56.9/56.2 & \cellcolor{red!10.0} 73.1/72.9 & \cellcolor{green!20.0} 88.4/88.8 & \cellcolor{green!15.0} 63.6/63.9 & \cellcolor{red!35.0} 80.6/79.9 & \cellcolor{red!25.0} 83.3/82.8 & \cellcolor{red!5.0} 89.1/89.0 & \cellcolor{red!50.0} 72.2/71.2 & \cellcolor{red!20.0} 83.0/82.6\\ 
ro & ro & \cellcolor{red!35.0} 55.8/55.1 & \cellcolor{green!35.0} 64.9/65.6 & \cellcolor{green!20.0} 80.3/80.7 & \cellcolor{green!30.0} 58.3/58.9 & \cellcolor{green!35.0} 72.2/72.9 & \cellcolor{green!15.0} 76.5/76.8 & \cellcolor{green!15.0} 89.2/89.5 & \cellcolor{green!15.0} 74.6/74.9 & \cellcolor{red!25.0} 81.6/81.1\\ 
ru & ru & \cellcolor{red!80.0} 44.0/42.4 & \cellcolor{green!90.0} 65.2/67.0 & \cellcolor{green!35.0} 85.8/86.5 & \cellcolor{green!15.0} 56.0/56.3 & \cellcolor{green!30.0} 71.0/71.6 & \cellcolor{red!10.0} 69.3/69.1 & \cellcolor{green!60.0} 82.6/83.8 & \cellcolor{red!10.0} 77.5/77.3 & \cellcolor{red!40.0} 76.4/75.6\\ 
ru & ru\_pud & \cellcolor{green!15.0} 55.9/56.2 & \cellcolor{green!25.0} 69.9/70.4 & \cellcolor{green!40.0} 90.3/91.1 & \cellcolor{red!5.0} 68.5/68.4 & \cellcolor{green!75.0} 76.3/77.8 & \cellcolor{green!15.0} 84.6/84.9 & \cellcolor{green!55.0} 90.0/91.1 & \cellcolor{green!25.0} 76.2/76.7 & \cellcolor{red!15.0} 84.4/84.1\\ 
ru & ru\_syntagrus & \cellcolor{green!0.0} 56.4/56.4 & \cellcolor{green!35.0} 65.1/65.8 & \cellcolor{green!40.0} 83.9/84.7 & \cellcolor{red!5.0} 57.2/57.1 & \cellcolor{green!55.0} 69.4/70.5 & \cellcolor{red!5.0} 74.7/74.6 & \cellcolor{green!40.0} 87.6/88.4 & \cellcolor{green!15.0} 75.0/75.3 & \cellcolor{red!15.0} 76.0/75.7\\ 
sk & sk & \cellcolor{red!40.0} 61.3/60.5 & \cellcolor{green!100} 76.6/79.1 & \cellcolor{red!10.0} 86.7/86.5 & \cellcolor{red!10.0} 68.6/68.4 & \cellcolor{red!25.0} 66.1/65.6 & \cellcolor{green!5.0} 74.6/74.7 & \cellcolor{green!5.0} 83.1/83.2 & \cellcolor{red!75.0} 78.0/76.5 & \cellcolor{red!10.0} 87.0/86.8\\ 
sl & sl & \cellcolor{green!35.0} 76.4/77.1 & \cellcolor{green!35.0} 68.4/69.1 & \cellcolor{green!5.0} 89.0/89.1 & \cellcolor{green!10.0} 72.8/73.0 & \cellcolor{green!0.0} 75.7/75.7 & \cellcolor{green!5.0} 78.7/78.8 & \cellcolor{red!15.0} 88.2/87.9 & \cellcolor{green!5.0} 78.2/78.3 & \cellcolor{red!10.0} 82.5/82.3\\ 
sl & sl\_sst & \cellcolor{green!100} 52.7/57.8 & \cellcolor{green!5.0} 58.4/58.5 & \cellcolor{green!25.0} 82.1/82.6 & \cellcolor{red!25.0} 46.3/45.8 & \cellcolor{green!100} 55.1/57.2 & \cellcolor{green!0.0} 64.8/64.8 & \cellcolor{red!40.0} 76.6/75.8 & \cellcolor{green!15.0} 64.1/64.4 & \cellcolor{red!15.0} 67.9/67.6\\ 
sv & sv & \cellcolor{red!15.0} 68.7/68.4 & \cellcolor{red!10.0} 68.9/68.7 & \cellcolor{green!15.0} 90.8/91.1 & \cellcolor{green!40.0} 68.8/69.6 & \cellcolor{red!5.0} 68.0/67.9 & \cellcolor{red!10.0} 85.3/85.1 & \cellcolor{green!45.0} 87.6/88.5 & \cellcolor{green!40.0} 68.3/69.1 & \cellcolor{green!10.0} 82.4/82.6\\ 
sv & sv\_lines & \cellcolor{red!25.0} 69.8/69.3 & \cellcolor{green!5.0} 73.8/73.9 & \cellcolor{green!35.0} 89.4/90.1 & \cellcolor{green!15.0} 66.3/66.6 & \cellcolor{red!15.0} 67.4/67.1 & \cellcolor{red!5.0} 86.7/86.6 & \cellcolor{green!15.0} 90.2/90.5 & \cellcolor{green!25.0} 75.1/75.6 & \cellcolor{green!25.0} 84.5/85.0\\ 
sv & sv\_pud & \cellcolor{red!35.0} 62.4/61.7 & \cellcolor{green!0.0} 75.0/75.0 & \cellcolor{green!25.0} 90.6/91.1 & \cellcolor{green!30.0} 68.8/69.4 & \cellcolor{red!15.0} 69.4/69.1 & \cellcolor{green!25.0} 85.0/85.5 & \cellcolor{green!30.0} 87.7/88.3 & \cellcolor{red!15.0} 72.5/72.2 & \cellcolor{green!20.0} 85.4/85.8\\ 
tr & tr & \cellcolor{red!100} 30.6/16.8 & \cellcolor{red!100} 49.6/46.6 & \cellcolor{green!80.0} 64.6/66.2 & \cellcolor{green!100.0} 29.5/31.5 & \cellcolor{red!100} 38.1/35.4 & \cellcolor{red!45.0} 55.4/54.5 & \cellcolor{green!100} 52.2/59.7 & \cellcolor{green!100} 45.0/49.6 & \cellcolor{green!100} 49.2/58.7\\ 
tr & tr\_pud & \cellcolor{red!100} 32.0/22.6 & \cellcolor{green!100} 34.2/38.5 & \cellcolor{green!100} 65.2/67.5 & \cellcolor{green!100} 29.5/35.4 & \cellcolor{green!100} 58.4/62.2 & \cellcolor{green!90.0} 39.8/41.6 & \cellcolor{green!100} 61.0/64.7 & \cellcolor{green!100} 56.0/61.5 & \cellcolor{green!100} 42.3/56.1\\ 
uk & uk & \cellcolor{green!35.0} 39.9/40.6 & \cellcolor{green!20.0} 70.6/71.0 & \cellcolor{green!20.0} 72.0/72.4 & \cellcolor{red!5.0} 52.9/52.8 & \cellcolor{green!100} 37.0/41.5 & \cellcolor{green!40.0} 67.4/68.2 & \cellcolor{red!15.0} 69.2/68.9 & \cellcolor{red!30.0} 61.2/60.6 & \cellcolor{red!35.0} 70.6/69.9\\ 
vi & vi & \cellcolor{green!60.0} 55.3/56.5 & \cellcolor{red!50.0} 65.1/64.1 & \cellcolor{green!100} 39.6/59.3 & \cellcolor{green!100} 35.6/38.1 & \cellcolor{green!100} 57.3/63.0 & \cellcolor{green!100} 50.0/52.5 & \cellcolor{green!100} 57.6/62.6 & \cellcolor{green!100} 46.6/51.4 & \cellcolor{green!85.0} 55.8/57.5\\ 
zh & zh & \cellcolor{red!100} 23.9/19.5 & \cellcolor{green!100} 66.4/70.8 & \cellcolor{green!100} 63.8/70.7 & \cellcolor{green!100} 25.4/29.9 & \cellcolor{green!100} 38.7/53.9 & \cellcolor{green!100} 32.4/39.9 & \cellcolor{green!85.0} 39.3/41.0 & \cellcolor{green!100} 47.6/50.7 & \cellcolor{green!100} 26.8/33.5 \\ \hline
    \end{tabular}
    \caption{Unlabeled attachment f-score of some of the frequent dependency relations for the baseline and the reordering ensemble model. We show the the two numbers separated by slash. We show the green color for improvement and the red color for worse result in the ensemble model; the darkness of the color indicates the level of difference.}
    \label{tab:dep_analysis}
\end{table*}

==> dominant_dir_gold.tex <==

\begin{figure}[t!]
    \centering
    \tiny
     \renewcommand{\arraystretch}{0.8}
     \setlength{\tabcolsep}{1.3pt}
    \begin{tabular}{cc c c c c c c c c c c c c c c c c c c}
       &  \begin{turn}{90}  acl  \end{turn} &  \begin{turn}{90}  advcl  \end{turn} &  \begin{turn}{90}  advmod  \end{turn} &  \begin{turn}{90}  amod  \end{turn} &  \begin{turn}{90}  appos  \end{turn} &  \begin{turn}{90}  aux  \end{turn} &  \begin{turn}{90}  ccomp  \end{turn} &  \begin{turn}{90}  cop  \end{turn} &  \begin{turn}{90}  csubj  \end{turn} &  \begin{turn}{90}  dislocated  \end{turn} &  \begin{turn}{90}  expl  \end{turn} &  \begin{turn}{90}  iobj  \end{turn} &  \begin{turn}{90}  nmod  \end{turn} &  \begin{turn}{90}  nsubj  \end{turn} &  \begin{turn}{90}  nummod  \end{turn} &  \begin{turn}{90}  obj  \end{turn} &  \begin{turn}{90}  obl  \end{turn} &  \begin{turn}{90}  vocative  \end{turn} &  \begin{turn}{90}  xcomp  \end{turn}  \\ 
ar & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
bg & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
cop & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
cs & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
da & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25} \\ 
de & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
el & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$ \\ 
en & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
es & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
et & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
eu & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$ \\ 
fa & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$ \\ 
fi & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
fr & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$ \\ 
he & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
hi & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$ \\ 
hr & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
hu & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$ \\ 
id & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
it & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$ \\ 
ja & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25} \\ 
ko & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25} \\ 
la & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25} \\ 
lt & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$ \\ 
lv & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
nl & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
no & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
pl & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
pt & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
ro & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
ru & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
sk & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
sl & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
sv & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
tr & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25} \\ 
uk & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
vi & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$ \\ 
zh & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{gray!25}  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{gray!25}  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{blue!25} $\rightarrow$  & \cellcolor{red!25} $\leftarrow$ 
    \end{tabular}
    \caption{A graphical depiction of dominant dependency order for different languages (the gray color shows no dominant order) based on the gold treebanks in the Bible data.}
    \label{fig:dominant_gold_info}
\end{figure}

==> dominant_dirs.tex <==
\begin{figure}[t!]
    \centering
    \tiny
     \renewcommand{\arraystretch}{0.5}
     \setlength{\tabcolsep}{.5pt}
    \begin{tabular}{cc c c c c c c c c c c c c c c c c c c}
    &  \begin{turn}{90}  acl  \end{turn} &  \begin{turn}{90}  advcl  \end{turn} &  \begin{turn}{90}  advmod  \end{turn} &  \begin{turn}{90}  amod  \end{turn} &  \begin{turn}{90}  appos  \end{turn} &  \begin{turn}{90}  aux  \end{turn} &  \begin{turn}{90}  ccomp  \end{turn} &  \begin{turn}{90}  cop  \end{turn} &  \begin{turn}{90}  csubj  \end{turn} &  \begin{turn}{90}  dislocated  \end{turn} &  \begin{turn}{90}  expl  \end{turn} &  \begin{turn}{90}  iobj  \end{turn} &  \begin{turn}{90}  nmod  \end{turn} &  \begin{turn}{90}  nsubj  \end{turn} &  \begin{turn}{90}  nummod  \end{turn} &  \begin{turn}{90}  obj  \end{turn} &  \begin{turn}{90}  obl  \end{turn} &  \begin{turn}{90}  vocative  \end{turn} &  \begin{turn}{90}  xcomp  \end{turn}  \\ 
ar & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
bg & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
cop & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
cs & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
da & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
de & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
el & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
en & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
es & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
et & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
eu & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25}\\ 
fa & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25}\\ 
fi & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
fr & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
he & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
hi & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25}\\ 
hr & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
hu & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
id & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
it & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
ja & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25}\\ 
ko & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25}\\ 
la & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
lt & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
lv & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
nl & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
no & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
pl & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
pt & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
ro & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
ru & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
sk & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
sl & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
sv & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
tr & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$\\ 
uk & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
vi & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$\\ 
zh & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{gray!25} & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{blue!25} $\rightarrow$ & \cellcolor{red!25} $\leftarrow$ & \cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{red!25} $\leftarrow$
    \end{tabular}
    \caption{A graphical depiction of dominant dependency direction for different languages (the gray color shows no dominant order) based on projected dependencies in the Bible data.}
    \label{fig:dominant_info}
\end{figure}


==> pos_dep_analysis.tex <==
\begin{table}[t!]
    \centering
    \tiny
     \renewcommand{\arraystretch}{0.5}
     \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{| l |l | c |c |c |c |c| c |}
    \hline
         lang & data & ADJ & ADV & NOUN & PRON & PROPN & VERB\\ \hline
ar & ar & \cellcolor{green!100} 74.3/77.8 & \cellcolor{red!100} 35.0/30.0 & \cellcolor{green!100} 58.1/60.7 & \cellcolor{green!100} 64.9/70.1 & \cellcolor{red!100} 15.7/11.8 & \cellcolor{green!100} 32.6/35.5\\ 
ar & ar\_pud & \cellcolor{green!100} 67.4/74.2 & \cellcolor{red!100} 24.9/21.2 & \cellcolor{green!100} 59.5/63.2 & \cellcolor{green!100} 65.5/70.7 & \cellcolor{green!0.0} 0.7/0.7 & \cellcolor{green!100} 55.0/59.4\\ 
bg & bg & \cellcolor{green!10.0} 90.6/90.8 & \cellcolor{green!15.0} 73.1/73.4 & \cellcolor{red!5.0} 78.5/78.4 & \cellcolor{green!25.0} 88.6/89.1 & \cellcolor{green!95.0} 80.0/81.9 & \cellcolor{green!0.0} 75.8/75.8\\ 
cop & cop & \cellcolor{green!0.0} 0.0/0.0 & \cellcolor{green!100} 48.0/53.8 & \cellcolor{green!100} 35.3/53.6 & \cellcolor{green!100} 68.4/83.3 & \cellcolor{green!100} 47.8/66.7 & \cellcolor{green!100} 37.4/44.0\\ 
cs & cs & \cellcolor{green!10.0} 85.2/85.4 & \cellcolor{green!0.0} 68.8/68.8 & \cellcolor{green!45.0} 66.2/67.1 & \cellcolor{red!15.0} 82.5/82.2 & \cellcolor{green!35.0} 68.9/69.6 & \cellcolor{green!10.0} 70.8/71.0\\ 
cs & cs\_cac & \cellcolor{green!15.0} 85.0/85.3 & \cellcolor{red!25.0} 66.6/66.1 & \cellcolor{green!45.0} 68.2/69.1 & \cellcolor{red!65.0} 83.3/82.0 & \cellcolor{green!60.0} 73.8/75.0 & \cellcolor{green!45.0} 71.3/72.2\\ 
cs & cs\_cltt & \cellcolor{red!10.0} 87.3/87.1 & \cellcolor{green!60.0} 50.8/52.0 & \cellcolor{green!80.0} 59.8/61.4 & \cellcolor{green!0.0} 76.9/76.9 & \cellcolor{green!100} 62.9/70.3 & \cellcolor{green!5.0} 56.9/57.0\\ 
cs & cs\_pud & \cellcolor{green!10.0} 85.5/85.7 & \cellcolor{red!20.0} 72.2/71.8 & \cellcolor{green!30.0} 68.0/68.6 & \cellcolor{red!75.0} 83.7/82.2 & \cellcolor{green!20.0} 74.3/74.7 & \cellcolor{green!0.0} 75.4/75.4\\ 
da & da & \cellcolor{green!25.0} 80.5/81.0 & \cellcolor{red!40.0} 71.4/70.6 & \cellcolor{red!10.0} 70.3/70.1 & \cellcolor{green!40.0} 82.4/83.2 & \cellcolor{green!0.0} 74.2/74.2 & \cellcolor{red!50.0} 64.4/63.4\\ 
de & de & \cellcolor{green!30.0} 81.6/82.2 & \cellcolor{green!30.0} 60.1/60.7 & \cellcolor{green!45.0} 66.4/67.3 & \cellcolor{green!25.0} 81.3/81.8 & \cellcolor{green!45.0} 67.1/68.0 & \cellcolor{red!60.0} 70.9/69.7\\ 
de & de\_pud & \cellcolor{green!40.0} 80.1/80.9 & \cellcolor{green!45.0} 61.9/62.8 & \cellcolor{green!25.0} 69.0/69.5 & \cellcolor{green!15.0} 87.1/87.4 & \cellcolor{green!10.0} 68.1/68.3 & \cellcolor{red!35.0} 74.5/73.8\\ 
el & el & \cellcolor{green!60.0} 84.2/85.4 & \cellcolor{red!55.0} 62.3/61.2 & \cellcolor{green!55.0} 64.3/65.4 & \cellcolor{red!95.0} 75.5/73.6 & \cellcolor{red!15.0} 66.9/66.6 & \cellcolor{green!20.0} 64.3/64.7\\ 
en & en & \cellcolor{green!15.0} 74.8/75.1 & \cellcolor{green!10.0} 72.8/73.0 & \cellcolor{green!0.0} 64.5/64.5 & \cellcolor{green!5.0} 85.7/85.8 & \cellcolor{green!10.0} 48.6/48.8 & \cellcolor{green!10.0} 71.1/71.3\\ 
en & en\_lines & \cellcolor{red!5.0} 82.6/82.5 & \cellcolor{green!5.0} 68.3/68.4 & \cellcolor{green!25.0} 69.0/69.5 & \cellcolor{green!20.0} 86.8/87.2 & \cellcolor{green!15.0} 70.5/70.8 & \cellcolor{green!45.0} 72.7/73.6\\ 
en & en\_partut & \cellcolor{green!35.0} 83.5/84.2 & \cellcolor{green!25.0} 71.8/72.3 & \cellcolor{green!25.0} 68.8/69.3 & \cellcolor{green!10.0} 86.4/86.6 & \cellcolor{green!0.0} 62.2/62.2 & \cellcolor{red!30.0} 71.7/71.1\\ 
en & en\_pud & \cellcolor{green!20.0} 79.1/79.5 & \cellcolor{green!15.0} 73.8/74.1 & \cellcolor{green!35.0} 69.2/69.9 & \cellcolor{green!5.0} 89.1/89.2 & \cellcolor{green!0.0} 60.3/60.3 & \cellcolor{green!20.0} 74.0/74.4\\ 
es & es & \cellcolor{green!10.0} 87.0/87.2 & \cellcolor{green!50.0} 75.8/76.8 & \cellcolor{green!15.0} 76.6/76.9 & \cellcolor{green!0.0} 85.7/85.7 & \cellcolor{green!20.0} 79.3/79.7 & \cellcolor{red!15.0} 64.9/64.6\\ 
es & es\_ancora & \cellcolor{green!5.0} 84.4/84.5 & \cellcolor{red!65.0} 74.6/73.3 & \cellcolor{green!0.0} 76.2/76.2 & \cellcolor{red!10.0} 86.9/86.7 & \cellcolor{green!5.0} 81.8/81.9 & \cellcolor{red!40.0} 68.8/68.0\\ 
es & es\_pud & \cellcolor{green!0.0} 87.6/87.6 & \cellcolor{red!100} 70.1/67.9 & \cellcolor{green!10.0} 78.4/78.6 & \cellcolor{green!10.0} 87.7/87.9 & \cellcolor{red!10.0} 81.5/81.3 & \cellcolor{green!30.0} 71.4/72.0\\ 
et & et & \cellcolor{green!25.0} 68.8/69.3 & \cellcolor{red!10.0} 65.7/65.5 & \cellcolor{green!0.0} 65.6/65.6 & \cellcolor{red!30.0} 71.8/71.2 & \cellcolor{red!40.0} 64.8/64.0 & \cellcolor{green!30.0} 64.5/65.1\\ 
eu & eu & \cellcolor{red!100} 56.3/53.9 & \cellcolor{green!100} 54.0/57.0 & \cellcolor{green!100} 31.9/52.5 & \cellcolor{green!100} 54.3/65.2 & \cellcolor{green!100} 42.4/54.1 & \cellcolor{green!100} 37.2/43.7\\ 
fa & fa & \cellcolor{green!100} 70.1/72.8 & \cellcolor{green!100} 43.8/48.3 & \cellcolor{green!100} 53.9/57.8 & \cellcolor{green!100} 66.5/70.0 & \cellcolor{green!0.0} 0.0/0.0 & \cellcolor{green!100} 51.7/56.0\\ 
fi & fi & \cellcolor{green!55.0} 74.2/75.3 & \cellcolor{green!30.0} 58.4/59.0 & \cellcolor{green!20.0} 59.0/59.4 & \cellcolor{red!25.0} 73.4/72.9 & \cellcolor{green!50.0} 68.9/69.9 & \cellcolor{red!10.0} 64.1/63.9\\ 
fi & fi\_ftb & \cellcolor{green!40.0} 74.2/75.0 & \cellcolor{green!30.0} 64.2/64.8 & \cellcolor{green!25.0} 64.2/64.7 & \cellcolor{red!40.0} 73.6/72.8 & \cellcolor{green!20.0} 64.5/64.9 & \cellcolor{green!30.0} 63.0/63.6\\ 
fi & fi\_pud & \cellcolor{green!40.0} 76.8/77.6 & \cellcolor{green!30.0} 63.1/63.7 & \cellcolor{green!15.0} 60.5/60.8 & \cellcolor{green!5.0} 78.3/78.4 & \cellcolor{green!35.0} 66.9/67.6 & \cellcolor{green!15.0} 69.4/69.7\\ 
fr & fr & \cellcolor{green!5.0} 86.6/86.7 & \cellcolor{green!5.0} 73.6/73.7 & \cellcolor{green!40.0} 74.5/75.3 & \cellcolor{green!40.0} 85.3/86.1 & \cellcolor{green!5.0} 79.4/79.5 & \cellcolor{green!20.0} 67.7/68.1\\ 
fr & fr\_partut & \cellcolor{red!5.0} 86.7/86.6 & \cellcolor{green!25.0} 76.5/77.0 & \cellcolor{green!35.0} 75.9/76.6 & \cellcolor{green!15.0} 83.3/83.6 & \cellcolor{red!10.0} 85.8/85.6 & \cellcolor{green!100.0} 68.1/70.1\\ 
fr & fr\_pud & \cellcolor{green!0.0} 87.1/87.1 & \cellcolor{red!20.0} 73.0/72.6 & \cellcolor{green!15.0} 77.3/77.6 & \cellcolor{green!5.0} 84.6/84.7 & \cellcolor{green!15.0} 79.9/80.2 & \cellcolor{red!15.0} 71.5/71.2\\ 
fr & fr\_sequoia & \cellcolor{green!0.0} 86.1/86.1 & \cellcolor{green!25.0} 72.1/72.6 & \cellcolor{red!10.0} 72.7/72.5 & \cellcolor{red!25.0} 84.7/84.2 & \cellcolor{green!25.0} 80.7/81.2 & \cellcolor{green!10.0} 69.5/69.7\\ 
he & he & \cellcolor{green!100} 74.7/77.5 & \cellcolor{green!100} 51.1/53.6 & \cellcolor{green!100} 62.8/65.7 & \cellcolor{green!100} 81.0/85.1 & \cellcolor{green!100} 66.8/69.5 & \cellcolor{green!95.0} 53.3/55.2\\ 
hi & hi & \cellcolor{green!45.0} 59.7/60.6 & \cellcolor{red!100} 52.0/47.8 & \cellcolor{green!70.0} 56.8/58.2 & \cellcolor{red!45.0} 63.5/62.6 & \cellcolor{red!100} 53.4/50.2 & \cellcolor{red!75.0} 50.8/49.3\\ 
hi & hi\_pud & \cellcolor{green!20.0} 63.2/63.6 & \cellcolor{green!100} 44.9/48.5 & \cellcolor{green!75.0} 51.0/52.5 & \cellcolor{green!20.0} 62.4/62.8 & \cellcolor{green!40.0} 52.2/53.0 & \cellcolor{green!5.0} 45.8/45.9\\ 
hr & hr & \cellcolor{green!0.0} 86.2/86.2 & \cellcolor{green!40.0} 67.9/68.7 & \cellcolor{green!40.0} 74.6/75.4 & \cellcolor{green!15.0} 83.5/83.8 & \cellcolor{green!40.0} 74.6/75.4 & \cellcolor{green!65.0} 72.2/73.5\\ 
hu & hu & \cellcolor{green!55.0} 78.7/79.8 & \cellcolor{green!0.0} 70.7/70.7 & \cellcolor{green!90.0} 64.1/65.9 & \cellcolor{green!0.0} 72.7/72.7 & \cellcolor{green!30.0} 58.1/58.7 & \cellcolor{red!35.0} 60.4/59.7\\ 
id & id & \cellcolor{green!100} 64.0/71.0 & \cellcolor{green!100} 78.2/80.9 & \cellcolor{green!100} 65.3/70.0 & \cellcolor{green!80.0} 89.7/91.3 & \cellcolor{green!100} 69.3/71.9 & \cellcolor{red!55.0} 65.2/64.1\\ 
it & it & \cellcolor{green!30.0} 84.9/85.5 & \cellcolor{green!100} 73.3/75.5 & \cellcolor{green!0.0} 77.7/77.7 & \cellcolor{red!15.0} 81.4/81.1 & \cellcolor{red!25.0} 79.7/79.2 & \cellcolor{red!25.0} 75.9/75.4\\ 
it & it\_pud & \cellcolor{green!10.0} 87.3/87.5 & \cellcolor{green!15.0} 77.7/78.0 & \cellcolor{green!5.0} 82.4/82.5 & \cellcolor{green!0.0} 88.3/88.3 & \cellcolor{green!0.0} 81.4/81.4 & \cellcolor{red!25.0} 77.8/77.3\\ 
ja & ja & \cellcolor{green!30.0} 56.6/57.2 & \cellcolor{red!5.0} 68.9/68.8 & \cellcolor{green!30.0} 61.2/61.8 & \cellcolor{red!60.0} 62.5/61.3 & \cellcolor{red!60.0} 64.2/63.0 & \cellcolor{red!45.0} 25.3/24.4\\ 
ja & ja\_pud & \cellcolor{green!75.0} 59.1/60.6 & \cellcolor{green!100} 63.2/67.4 & \cellcolor{green!5.0} 58.1/58.2 & \cellcolor{green!100} 64.6/66.9 & \cellcolor{green!0.0} 59.9/59.9 & \cellcolor{green!15.0} 29.6/29.9\\ 
ko & ko & \cellcolor{red!90.0} 69.1/67.3 & \cellcolor{green!100.0} 53.5/55.5 & \cellcolor{green!35.0} 35.8/36.5 & \cellcolor{green!100} 43.6/46.2 & \cellcolor{green!0.0} 0.0/0.0 & \cellcolor{green!100.0} 43.4/45.4\\ 
la & la & \cellcolor{green!100} 46.4/48.5 & \cellcolor{red!35.0} 61.5/60.8 & \cellcolor{red!30.0} 54.3/53.7 & \cellcolor{red!45.0} 63.1/62.2 & \cellcolor{red!10.0} 67.5/67.3 & \cellcolor{red!10.0} 49.1/48.9\\ 
la & la\_ittb & \cellcolor{green!0.0} 65.4/65.4 & \cellcolor{red!10.0} 64.9/64.7 & \cellcolor{green!95.0} 55.0/56.9 & \cellcolor{red!20.0} 64.9/64.5 & \cellcolor{red!25.0} 52.7/52.2 & \cellcolor{red!25.0} 50.4/49.9\\ 
la & la\_proiel & \cellcolor{green!5.0} 67.5/67.6 & \cellcolor{green!5.0} 55.1/55.2 & \cellcolor{red!15.0} 59.4/59.1 & \cellcolor{green!0.0} 74.4/74.4 & \cellcolor{red!5.0} 58.9/58.8 & \cellcolor{red!10.0} 57.4/57.2\\ 
lt & lt & \cellcolor{red!40.0} 68.3/67.5 & \cellcolor{red!75.0} 71.3/69.8 & \cellcolor{green!55.0} 63.6/64.7 & \cellcolor{red!90.0} 70.2/68.4 & \cellcolor{green!100.0} 66.7/68.7 & \cellcolor{green!0.0} 55.9/55.9\\ 
lv & lv & \cellcolor{green!45.0} 64.0/64.9 & \cellcolor{green!25.0} 72.0/72.5 & \cellcolor{red!10.0} 56.7/56.5 & \cellcolor{green!15.0} 71.1/71.4 & \cellcolor{red!40.0} 61.6/60.8 & \cellcolor{green!25.0} 63.9/64.4\\ 
nl & nl & \cellcolor{green!100} 74.7/77.5 & \cellcolor{red!25.0} 60.1/59.6 & \cellcolor{green!25.0} 65.1/65.6 & \cellcolor{red!15.0} 75.5/75.2 & \cellcolor{green!15.0} 61.2/61.5 & \cellcolor{green!15.0} 52.7/53.0\\ 
nl & nl\_lassysmall & \cellcolor{green!30.0} 77.2/77.8 & \cellcolor{green!55.0} 70.6/71.7 & \cellcolor{green!5.0} 69.3/69.4 & \cellcolor{green!50.0} 86.7/87.7 & \cellcolor{red!20.0} 76.2/75.8 & \cellcolor{green!20.0} 72.6/73.0\\ 
no & no\_bokmaal & \cellcolor{green!15.0} 80.5/80.8 & \cellcolor{green!10.0} 73.5/73.7 & \cellcolor{green!15.0} 75.8/76.1 & \cellcolor{red!15.0} 86.3/86.0 & \cellcolor{red!15.0} 72.1/71.8 & \cellcolor{green!10.0} 73.6/73.8\\ 
no & no\_nynorsk & \cellcolor{green!45.0} 77.1/78.0 & \cellcolor{green!25.0} 62.3/62.8 & \cellcolor{green!30.0} 71.0/71.6 & \cellcolor{green!15.0} 79.2/79.5 & \cellcolor{red!5.0} 72.3/72.2 & \cellcolor{green!15.0} 68.4/68.7\\ 
pl & pl & \cellcolor{green!30.0} 76.7/77.3 & \cellcolor{green!45.0} 80.6/81.5 & \cellcolor{green!0.0} 74.5/74.5 & \cellcolor{red!5.0} 87.9/87.8 & \cellcolor{green!15.0} 76.3/76.6 & \cellcolor{red!5.0} 86.7/86.6\\ 
pt & pt & \cellcolor{red!15.0} 85.0/84.7 & \cellcolor{green!20.0} 69.5/69.9 & \cellcolor{green!0.0} 77.8/77.8 & \cellcolor{green!15.0} 81.1/81.4 & \cellcolor{red!10.0} 82.8/82.6 & \cellcolor{red!45.0} 70.5/69.6\\ 
pt & pt\_br & \cellcolor{green!15.0} 79.9/80.2 & \cellcolor{green!10.0} 72.0/72.2 & \cellcolor{red!10.0} 75.9/75.7 & \cellcolor{green!5.0} 81.1/81.2 & \cellcolor{green!5.0} 73.8/73.9 & \cellcolor{red!25.0} 63.1/62.6\\ 
pt & pt\_pud & \cellcolor{green!10.0} 83.3/83.5 & \cellcolor{green!0.0} 71.9/71.9 & \cellcolor{red!25.0} 77.0/76.5 & \cellcolor{green!0.0} 79.5/79.5 & \cellcolor{red!30.0} 83.5/82.9 & \cellcolor{green!5.0} 69.3/69.4\\ 
ro & ro & \cellcolor{green!40.0} 79.2/80.0 & \cellcolor{green!30.0} 62.9/63.5 & \cellcolor{green!15.0} 71.2/71.5 & \cellcolor{green!10.0} 83.0/83.2 & \cellcolor{red!10.0} 81.2/81.0 & \cellcolor{red!40.0} 69.0/68.2\\ 
ru & ru & \cellcolor{green!10.0} 81.9/82.1 & \cellcolor{green!100} 62.5/64.9 & \cellcolor{green!25.0} 67.9/68.4 & \cellcolor{red!35.0} 74.0/73.3 & \cellcolor{green!10.0} 73.0/73.2 & \cellcolor{red!40.0} 73.3/72.5\\ 
ru & ru\_pud & \cellcolor{green!0.0} 89.1/89.1 & \cellcolor{green!35.0} 70.5/71.2 & \cellcolor{green!50.0} 76.7/77.7 & \cellcolor{green!65.0} 86.2/87.5 & \cellcolor{green!40.0} 79.4/80.2 & \cellcolor{green!5.0} 73.8/73.9\\ 
ru & ru\_syntagrus & \cellcolor{green!0.0} 83.1/83.1 & \cellcolor{green!40.0} 62.9/63.7 & \cellcolor{green!40.0} 70.4/71.2 & \cellcolor{green!0.0} 78.3/78.3 & \cellcolor{green!25.0} 75.7/76.2 & \cellcolor{red!20.0} 65.9/65.5\\ 
sk & sk & \cellcolor{green!5.0} 85.0/85.1 & \cellcolor{green!65.0} 84.2/85.5 & \cellcolor{red!20.0} 74.2/73.8 & \cellcolor{red!100.0} 92.1/90.1 & \cellcolor{green!5.0} 59.1/59.2 & \cellcolor{red!25.0} 86.1/85.6\\ 
sl & sl & \cellcolor{red!5.0} 86.1/86.0 & \cellcolor{green!30.0} 77.6/78.2 & \cellcolor{green!15.0} 76.8/77.1 & \cellcolor{red!25.0} 85.3/84.8 & \cellcolor{red!20.0} 82.1/81.7 & \cellcolor{red!20.0} 80.5/80.1\\ 
sl & sl\_sst & \cellcolor{green!15.0} 72.1/72.4 & \cellcolor{green!10.0} 57.7/57.9 & \cellcolor{red!10.0} 62.0/61.8 & \cellcolor{green!50.0} 71.7/72.7 & \cellcolor{green!100} 38.8/42.0 & \cellcolor{green!10.0} 57.1/57.3\\ 
sv & sv & \cellcolor{green!15.0} 86.2/86.5 & \cellcolor{red!15.0} 66.1/65.8 & \cellcolor{green!20.0} 73.2/73.6 & \cellcolor{green!15.0} 86.0/86.3 & \cellcolor{red!25.0} 69.0/68.5 & \cellcolor{red!15.0} 74.6/74.3\\ 
sv & sv\_lines & \cellcolor{green!35.0} 85.9/86.6 & \cellcolor{red!10.0} 72.0/71.8 & \cellcolor{green!20.0} 75.9/76.3 & \cellcolor{red!15.0} 87.1/86.8 & \cellcolor{green!45.0} 71.9/72.8 & \cellcolor{red!15.0} 75.0/74.7\\ 
sv & sv\_pud & \cellcolor{green!15.0} 86.9/87.2 & \cellcolor{green!0.0} 72.4/72.4 & \cellcolor{green!10.0} 75.3/75.5 & \cellcolor{green!35.0} 88.7/89.4 & \cellcolor{green!0.0} 62.6/62.6 & \cellcolor{green!20.0} 76.3/76.7\\ 
tr & tr & \cellcolor{green!100} 56.4/58.9 & \cellcolor{green!100} 54.2/56.3 & \cellcolor{green!90.0} 46.5/48.3 & \cellcolor{red!5.0} 56.0/55.9 & \cellcolor{green!20.0} 44.6/45.0 & \cellcolor{green!100} 38.0/45.8\\ 
tr & tr\_pud & \cellcolor{green!65.0} 57.3/58.6 & \cellcolor{green!100} 38.6/43.5 & \cellcolor{green!100} 44.5/48.1 & \cellcolor{green!100} 45.6/50.1 & \cellcolor{green!100} 40.2/42.4 & \cellcolor{green!100} 42.9/54.6\\ 
uk & uk & \cellcolor{green!5.0} 70.6/70.7 & \cellcolor{green!10.0} 64.8/65.0 & \cellcolor{green!45.0} 54.5/55.4 & \cellcolor{green!65.0} 72.0/73.3 & \cellcolor{green!0.0} 0.0/0.0 & \cellcolor{red!15.0} 60.0/59.7\\ 
vi & vi & \cellcolor{green!100} 40.7/50.2 & \cellcolor{green!0.0} 0.0/0.0 & \cellcolor{green!100} 45.1/50.4 & \cellcolor{green!0.0} 0.0/0.0 & \cellcolor{green!100} 58.0/60.6 & \cellcolor{green!100} 43.5/46.9\\ 
zh & zh & \cellcolor{green!100} 55.0/59.1 & \cellcolor{green!100} 63.0/68.7 & \cellcolor{green!100} 42.4/48.0 & \cellcolor{green!90.0} 56.0/57.8 & \cellcolor{green!100} 37.1/41.3 & \cellcolor{green!100.0} 23.9/25.9\\ \hline
    \end{tabular}
    \caption{Unlabeled attachment f-score of POS tags as dependents for the baseline and the reordering ensemble model. We show the the two numbers separated by slash, the green color for improvement, and the red color for worse result in the ensemble model; the darkness of the color indicates the level of difference.}
    \label{tab:dep_pos_analysis}
\end{table}

==> proj_stat.tex <==
\begin{table}[t!]
    \centering
\scriptsize
     \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{c|c c c}
    \hline \hline
        L. & Sen. & Len. & Density \\  \hline
ar & 985 & 19.1 & 0.58 \\ 
bg & 11546 & 27.7 & 0.75 \\ 
cop & 2 & 2.0 & 1.00 \\ 
cs & 138 & 25.0 & 0.41 \\ 
da & 9955 & 23.9 & 0.73 \\ 
de & 15181 & 28.0 & 0.75 \\ 
el & 3428 & 27.7 & 0.64 \\ 
en & 44576 & 28.7 & 0.85 \\ 
es & 20811 & 26.8 & 0.80 \\ 
et & 881 & 22.7 & 0.59 \\ 
eu & 171 & 20.9 & 0.62 \\ 
fa & 3688 & 27.4 & 0.61 \\ 
fi & 10240 & 25.1 & 0.74 \\ 
fr & 20316 & 28.1 & 0.82 \\ 
he & 1623 & 21.3 & 0.63 \\ 
hi & 2539 & 30.0 & 0.54 \\ 
hr & 9363 & 25.4 & 0.73 \\ 
hu & 1165 & 29.2 & 0.57 \\ 
id & 1557 & 27.4 & 0.53 \\ 
it & 16599 & 27.4 & 0.77 \\ 
ja & 604 & 33.5 & 0.48 \\ 
ko & 447 & 15.2 & 0.61 \\ 
la & 10442 & 19.9 & 0.77 \\ 
lt & 3945 & 22.5 & 0.68 \\ 
lv & 2774 & 22.2 & 0.76 \\ 
nl & 3155 & 30.7 & 0.55 \\ 
no & 20807 & 27.1 & 0.83 \\ 
pl & 10875 & 25.9 & 0.75 \\ 
pt & 140 & 32.6 & 0.49 \\ 
ro & 11443 & 28.7 & 0.72 \\ 
ru & 13853 & 24.8 & 0.77 \\ 
sk & 16269 & 25.6 & 0.78 \\ 
sl & 14139 & 26.6 & 0.76 \\ 
sv & 18373 & 27.7 & 0.79 \\ 
tr & 310 & 20.7 & 0.52 \\ 
uk & 463 & 23.6 & 0.63 \\ 
vi & 773 & 31.5 & 0.53 \\ 
zh & 181 & 33.0 & 0.46 \\\hline
Avg. & 7994	& 25	& 0.7 \\
\hline \hline
    \end{tabular}
    \caption{Statistics of the projected dependencies in the Bible data after applying the density filter. The second column shows the number of sentences, the third column shows the average sentence length, and the last column shows the proportion of projected dependencies with respect to the number of words in the sentences.}
    \label{tab:proj_stats}
\end{table}

==> reorder_algo.tex <==
\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LState{\State \algbackskip}%
\makeatother

\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LComment{\Comment \algbackskip}%
\makeatother
\newcommand{\var}{\texttt}
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{figure}[t!]
\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\vspace{0.2cm}
%\noindent\rule{0.5\textwidth}{0.4pt}
\begin{algorithmic}[0]
\small
 \LState {{\bf Inputs: }{1) Source treebank $\mathcal{D}$ with the dominant order values $\lambda^{\mathcal{D}}$, 2) Dominant dependencies $\lambda^{(\allproj)}$ from projected dependencies $\allproj$ for the target language, 3) Set of dependency labels for reordering $\mathcal{L}$.}}
\vspace{0.2cm}
 \Function{ReorderTree}{\var{$\mathcal{D}$}, \var{i}, \var{h}}
 \State {final\_order = []}
 \State {before\_head = [], after\_head = []}
  \ForEach {$j ~{\tt in}~ {\tt sorted(dependents_t(h))}$}
  \If{$r^i_j \in \mathcal{L}$}
  \If{$\lambda^{(\mathcal{D})}(r^i_j, \delta^i_j) \neq \lambda^{(\allproj)}(r^i_j, \delta^i_j)$} 
  \If{$\lambda^{(\allproj)}(r^i_j, \overline{\delta^i_j}) = {\tt true}$}
  \State{Set $\delta^i_j = \overline{\delta^i_j}$}
   \EndIf
   \EndIf
   \EndIf
   \If{$\delta^i_j = \rightarrow$}
   \State{Append j to after\_head}
    \Else \State{Append j to before\_head}
    \EndIf
  \EndFor
  \ForEach {$c$ in before\_head}
  \State{c\_order = ReorderTree(\var{$\mathcal{D}$}, \var{i}, \var{c}})
  \State{Append c\_order to final\_order}
  \EndFor
     
     \State{Append {\bf h} to final\_order}
     
    \ForEach {$c$ in after\_head}
  \State{c\_order = ReorderTree(\var{$\mathcal{D}$}, \var{i}, \var{c}})
  \State{Append c\_order to final\_order}
  \EndFor
  
  \State{\Return{final\_order}}
  \EndFunction
  
\vspace{0.2cm}
\LState{\bf Algorithm:}
\State  Initialize $\mathcal{D}' = []$
\For {$i$ = 1 to $|\mathcal{D}|$}
\State{new\_order = ReorderTree(\var{$\mathcal{D}$}, \var{i}, 0)}
\State{$t'$ = Reorder $\mathcal{D}^i$ wrt new\_order}
\State{Append $t'$ to  $\mathcal{D}'$}
\EndFor

\State{\Return{ $\mathcal{D}'$}}
\end{algorithmic}

\vspace{0.2cm}

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\caption{Reordering algorithm for a source treebank.}\label{fig:reorder_alg}

\end{figure}

